Fat Tails and Black Swans: Exact Results for Multiplicative Processes with Resets

We consider a class of multiplicative processes which, added with stochastic reset events, give origin to stationary distributions with power-law tails -- ubiquitous in the statistics of social, economic, and ecological systems. Our main goal is to provide a series of exact results on the dynamics and asymptotic behaviour of increasingly complex versions of a basic multiplicative process with resets, including discrete and continuous-time variants and several degrees of randomness in the parameters that control the process. In particular, we show how the power-law distributions are built up as time elapses, how their moments behave with time, and how their stationary profiles become quantitatively determined by those parameters. Our discussion emphasizes the connection with financial systems, but these stochastic processes are also expected to be fruitful in modeling a wide variety of social and biological phenomena.

==> rev1.tex <==
San Carlos de Bariloche, February 7th 2020

Dear Editor,

Thank you for sending the reviewers' reports on the manuscript #CHA19-AR-DSS2020-01609 "Fat tails and black swans..." by myself and S. Manrubia. We are now submitting the revised version. Our responses to the reviewers' comments, as well as the detail of changes, follow this message.

Yours sincerely,

Damián Zanette

RESPONSES

Reviewer #1

> Importantly, I miss a reference and discussion of the paper of S. Redner... This 30-year old paper should not be ignored as it overlaps a lot with the present contribution. Also the review paper by Michael Mitzenmacher should be cited. 

Response: Redner's 1990 tutorial is indeed an important precedent to the discussion of extreme events and their role in the statistics of random multiplicative processes. It is now cited and commented in the second paragraph of section II.B, and cited again towards the end of the same section.  Mitzenmacher's review is also a useful reference, which we now cite in the introduction.

> As a physicists I would like to see some commet on what happens for these type of pre in spatially extended systems.  

Response: In the second-to-last paragraph of section V we now comment on the necessity of generalizing these processes to spatially extended systems, for application to problems of physical and biological origin. A thorough discussion of this generalization, however, exceeds the scope of our contribution.

> Typos: Pag 3... 

Response: The typo has been corrected. 

Reviewer #2

> ... Credit to this blossoming of interest about the consequences of introducing reset events in continuous or discrete random processes is usually granted to Refs. [1,2], respectively: [1] M. R. Evans and S. N. Majumdar, Phys. Rev. Lett. 106, 160601 (2011). [2] M. Montero and J. Villarroel, Phys. Rev. E 87, 012116 (2013).

Response: Although our discussion mainly frames stochastic multiplicative processes with resetting in the context of finance dynamics, we agree that the papers pointed out by the reviewer are important landmarks in the growing interest of the field. We have therefore added the references to our bibliography and cited them in section I.

> ... [3] M. Montero and J. Villarroel, Phys. Rev. E 94, 032132 (2016) ... I recommend that the authors carefully read the cited Ref. [3], and establish these (and maybe additional) connections between these two works.

Response: The reviewer is right that the system studied in this reference, although formulated and treated in a different way, bears substantial overlap with the special case considered in our section II. We now cite the reference and mention the connection with our Eqs. (1), (4), (5), (12) and (14). 

As a matter of fact, a remark by the reviewer on a discrepancy between our Eq. (14) and a result in the cited reference allowed us to detect an error in our calculations (without consequences for our conclusions), which has now been corrected. We thank the reviewer for pointing out this.


 

